LoLa: Low-Latency Realtime Video Conferencing over Multiple Cellular Carriers

LoLa is a novel multi-path system for video conferencing applications over cellular networks. It provides significant gains over single link solutions when the link quality over different cellular networks fluctuate dramatically and independently over time, or when aggregating the throughput across different cellular links improves the perceived video quality. LoLa achieves this by continuously estimating the quality of available cellular links to decide how to strip video packets across them without inducing delays or packet drops. It is also tightly coupled with state-of-the-art video codec to dynamically adapt video frame size to respond quickly to changing network conditions. Using multiple traces collected over 4 different cellular operators in a large metropolitan city, we demonstrate that LoLa provides significant gains in terms of throughput and delays compared to state-of-the-art real-time video conferencing solution.

==> Makefile <==
REPORT=paper
FIGS=$(wildcard figures/*.pdf)

REPORT_PDF = $(REPORT:%=%.pdf)
REPORT_BBL = $(REPORT:%=%.bbl)
REPORT_SRC = $(REPORT:%=%.tex)
REFS=$(wildcard *.bib)
CLASSFILES=$(wildcard *.cls) $(wildcard *.sty)
NOTSRCS=$(REPORT:%=%.tex)
SRCS=$(filter-out $(NOTSRCS),$(wildcard *.tex)) $(CLASSFILES)

LATEX=pdflatex
BIBTEX=bibtex
LATEXOPTS=
PS2PDF=epstopdf
THUMBPDF=thumbpdf

all: $(REPORT_PDF)

$(REPORT_BBL): %.bbl: %.bib
	$(LATEX) $(LATEXOPTS) $(REPORT)
	$(BIBTEX) $(REPORT)

$(REPORT_PDF): %.pdf: %.tex %.bbl $(SRCS) $(REFS) $(FIGS) $(CLASSFILES)
	$(BIBTEX) $*
	while ($(LATEX) $(LATEXOPTS) $< ; \
    grep -q "Rerun to get" $*.log ) do true ; \
    done

clean:
	rm -f *.out *.bak *.dvi \
        *.aux *.log *.blg *.bbl \
  $(REPORT_PDF)


==> packages.tex <==
\usepackage{balance}
\usepackage{tabulary}
\usepackage{ifthen}
\usepackage[font=small,format=plain,labelfont=bf,textfont=it,aboveskip=3pt,belowskip=3pt]{caption}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{enumitem}
\usepackage{pifont}
\usepackage{fancyhdr}
\usepackage{cite}
\usepackage{booktabs}
\usepackage{color}
\usepackage{colortbl}
\usepackage{courier}
\usepackage[scaled=0.92]{helvet}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{listings}
\usepackage{tikz}
\usepackage[absolute]{textpos}
\usepackage{multirow}
\usepackage{xspace}
\usepackage[english]{babel}
\usepackage{blindtext}
\usepackage{epsfig,endnotes,siunitx,subcaption,times}
\usepackage{tabularx}
\usepackage{array}
\usepackage{bm}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{appendix}
\usepackage{wasysym}
\usepackage{algpseudocode}
\usepackage[ruled, linesnumbered, noend]{algorithm2e}
\usepackage[filecolor=black,citecolor=blue,urlcolor=black,linkcolor=blue,colorlinks,pdfpagelabels,pdfpagelayout=SinglePage]{hyperref}

%%%%%%%%%%%%%
% Space hacks
\usepackage{microtype}
\usepackage[compact]{titlesec} % SPACE
\addtolength{\textfloatsep}{-12pt} % SPACE
\setlist{itemsep=0pt,parsep=0pt} % more compact lists

%\usepackage{titling}
%\setlength{\droptitle}{-2cm}
\date{}

